Evaluation of Distimation's Real-world Performance on a Superconducting Quantum Computer

Quantum state estimation plays a crucial role in ensuring reliable creation of entanglement within quantum networks, yet conventional Quantum State Tomography (QST) methods remain resource-intensive and impractical for scaling. To address these limitations, we experimentally validate Distimation, a novel distillation-based protocol designed for efficient Bell-diagonal state estimation. Using IBM Quantum simulators and hardware, we demonstrate that Distimation accurately estimates Bell parameters under simulated and real-world noise conditions, but also demonstrating limitations with operational noise and number of available shots. Additionally, we simulate an asymmetric-fidelity Bell pair scenario via Measurement-Based Quantum Computation (MBQC) to further validate Distimation under realistic network conditions. Our results establish Distimation as a viable method for scalable, real-time entanglement monitoring in practical quantum networks.

==> adaptive-distimation.tex <==
While Phase 1 validated Distimation for static Bell-diagonal states, practical quantum networks often operate in dynamic environments where noise parameters drift over time. In Phase 2, we extend Distimation to an adaptive Bayesian framework that can continuously track such time-varying Pauli error parameters.

\subsection{Problem Formulation}

We consider a Bell-diagonal channel subject to slowly varying Pauli noise:
\[
\mathcal{E}_t(\rho) = (1 - p_x(t) - p_y(t) - p_z(t)) \rho + \sum_{i \in \{x,y,z\}} p_i(t) (\sigma_i \otimes \sigma_i) \rho (\sigma_i \otimes \sigma_i)
\]
where each \( p_i(t) \) varies sinusoidally over time.

The task is to estimate the current values of \( \vec{p}_t = (p_x, p_y, p_z) \) using only the measurement outcomes of the three distillation circuits at each time step.

\subsection{Bayesian Estimator Design}

We model the posterior distribution over \( \vec{p}_t \) on a discretized 3D grid. At each time step, the prior \( P(\vec{p}_{t-1}) \) is updated based on observed data \( D_t \) using Bayes' rule:
\[
P(\vec{p}_t \mid D_t) \propto \mathcal{L}(D_t \mid \vec{p}_t) \cdot P(\vec{p}_{t-1})
\]
We assume a uniform prior at \( t = 0 \). The likelihood \( \mathcal{L}(D_t | \vec{p}) \) is modeled as a product of binomial distributions derived from the success outcomes (``00'' and ``11'') of each purification basis (X, Z, Y).

To ensure numerical stability over long runs, we evaluate the log-likelihood:
\[
\log \mathcal{L}(D_t | \vec{p}) = \sum_{i} \left[ k_i \log p_i + (N - k_i) \log(1 - p_i) \right]
\]
where \( k_i \) is the number of successful outcomes and \( N \) is the number of shots per circuit.

After computing and normalizing the posterior, the maximum a posteriori (MAP) estimate is selected as:
\[
\hat{\vec{p}}_t = \arg\max_{\vec{p}} P(\vec{p}_t | D_{1:t})
\]

\subsection{Simulation Setup}

We simulate 50 time steps using Qiskit's AerSimulator. At each step:
\begin{enumerate}
    \item The true noise parameters \( (p_x, p_y, p_z) \) are generated with sinusoidal variation.
    \item All three distillation circuits are executed with 1,000 shots each.
    \item The posterior distribution is updated on a grid of size \( 25 \times 25 \times 25 \).
    \item Estimated parameters are recorded and compared against ground truth.
\end{enumerate}

\subsection{Results and Discussion}

Figure~\ref{fig:adaptive-tracking} shows the true vs. estimated Pauli error parameters over time. The Bayesian estimator successfully tracks the underlying drift across all axes. Notably, it adapts to changes in \( p_z(t) \), which had previously failed in naive averaging schemes. The tracking performance is visualized below.

\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{image/adaptive_tracking_plot.png}
\caption{Bayesian tracking of time-varying Pauli noise. Dashed lines show true values; solid lines show MAP estimates.}
\label{fig:adaptive-tracking}
\end{figure}

While tracking performance depends on the grid resolution and shot count, this experiment demonstrates the viability of non-tomographic Bayesian state tracking using only three measurement bases. Future work may consider:
\begin{itemize}
    \item Particle filtering for continuous posterior approximation
    \item Kalman-style recursive filters in the \((x_1, x_2, x_3)\) space
    \item Smoothing using past posteriors or expectation-maximization
\end{itemize}

This phase validates that Distimation can be extended from static to dynamic regimes, enabling lightweight, continuous entanglement characterization in evolving quantum systems.


In addition to visual alignment in Figure~\ref{fig:adaptive-tracking}, we quantify estimation accuracy using root-mean-square error (RMSE) between true and estimated parameters over 50 time steps:
\[
\text{RMSE}(p_x) = 0.0017, \quad \text{RMSE}(p_y) = 0.0017, \quad \text{RMSE}(p_z) = 0.0038
\]
These values confirm that the Bayesian estimator achieves high precision across all axes, with average absolute error below 0.4\% per timestep. The slight increase in \( p_z \) RMSE is consistent with its larger dynamic range in the underlying model.


==> bell-diagonal-parameter-estimation.tex <==
Evaluated the Bell Diagonal assumption in respect to the true noisy state by computing the trace distance. 

From Fig~\ref{Purification-Result} results, we calculated success probabilities \( \hat{p}^{(i)} \) and determined the intermediate parameters \( x_i \), leading to the following Bell-diagonal estimates, using Eq~\ref{eq:bd-intermediate-calculation}:
\[
\hat{q} = (0.743,\ 0.200,\ 0.032,\ 0.025)
\quad \text{with} \quad \sum \hat{q}_i = 1.00
\]
Using these Bell diagonal estimate, Bell diagonal state density matrix $\hat{\rho_{BD}}$ was constructed. Similar to the Werner Distimation, to quantitatively evaluate these results, we calculated the trace distance between the Distimation-estimated Bell Diagonal state \(\hat{\rho}_{BD}\) and the actual noisy state \(\rho_{\text{QST}}\), obtained through QST. Then, we computed the trace distance \(D(\hat{\rho}_{BD}, \rho_{\text{QST}})\) which was ....
